Survival Instinct in Offline Reinforcement Learning

We present a novel observation about the behavior of offline reinforcement learning (RL) algorithms: on many benchmark datasets, offline RL can produce well-performing and safe policies even when trained with "wrong" reward labels, such as those that are zero everywhere or are negatives of the true rewards. This phenomenon cannot be easily explained by offline RL's return maximization objective. Moreover, it gives offline RL a degree of robustness that is uncharacteristic of its online RL counterparts, which are known to be sensitive to reward design. We demonstrate that this surprising robustness property is attributable to an interplay between the notion of pessimism in offline RL algorithms and certain implicit biases in common data collection practices. As we prove in this work, pessimism endows the agent with a "survival instinct", i.e., an incentive to stay within the data support in the long term, while the limited and biased data coverage further constrains the set of survival policies. Formally, given a reward class -- which may not even contain the true reward -- we identify conditions on the training data distribution that enable offline RL to learn a near-optimal and safe policy from any reward within the class. We argue that the survival instinct should be taken into account when interpreting results from existing offline RL benchmarks and when creating future ones. Our empirical and theoretical results suggest a new paradigm for RL, whereby an agent is nudged to learn a desirable behavior with imperfect reward but purposely biased data coverage.

==> appendices/old_draft.tex <==
\section{Analysis \chingan{old draft}}



\subsection{Main Results}

Below we consider performing offline RL with rewards labeled by a reward function in a reward class $\tilde{\RR}$. Without loss of generality, we suppose $\tilde{r}(s,a)\in[0,1]$ for all $\tilde{r}\in\tilde{\RR}$. We do not assume $\tilde{\RR}$ contains the true reward function $r$.



\begin{definition}[Robustness of Distribution] \label{def:distribution robustness2}
    Let $\tilde{\RR}$ be a reward class of rewards in $[0,1]$.
    Given a distribution $\mu \in \Delta(\SS\times\AA)$ and $\tilde{r}\in\tilde{\RR}$, define a cost function 
    \begin{align*}
        c_\mu(s,a) \coloneqq \one[ \mu(s,a)= 0]
    \end{align*}
    and a constrained MDP $\CC_\mu(\tilde{r}) \coloneqq   \CC(\SS,\AA, \tilde{r},c_\mu,P,\gamma)$.
    %
    We say the distribution $\mu$ is $\frac{1}{\epsilon}$-\emph{robust} with respect to $\tilde{\RR}$ if, for all $\delta\geq 0$,
    \begin{align}
         \max_{\tilde{r}\in\tilde{\RR}} \max_{\pi \in  \Pi_\delta(\CC_\mu(\tilde{r}))} %V_r^{\pi^*}(d_0) -  V_r^{\pi}(d_0) 
         J(\pi^*) - J(\pi) 
         \leq \epsilon + O(\delta)
    \end{align}   
\end{definition}

\chingan{ Give motivation of this definition (connection to pessimism).}
\begin{remark}
    Some examples
    \begin{itemize}
        \item (Standard offline RL assumption) If $d^{\pi^*} \ll \mu$, then $\mu$ is $\infty$-robust to $\tilde{\RR} = \{  \bar{r} : \bar{r}(s,a) = C( r(s,a) + \E_{s'|s,a}[h(s')] - h(s)\}), C>0, h:\SS\to\R\}$.
        \item (Imitation Learning assumption) If $d^{\pi^*}=\mu$, then $\mu$ $\infty$-robust to $\tilde{\RR} = \{ \bar{r}: \bar{r}: \SS\times\AA\to\R\}$.

        \item \todo{} (Feasible Action) Suppose all actions $a$ in the support of $\mu(\cdot|s)$ satisfies $Q^*(s,a) \geq V^*(s) -\epsilon$. 
        Then $\mu$ is $\frac{1-\gamma}{\epsilon}$-robust to to $\tilde{\RR} = \{ \bar{r}: \bar{r}: \SS\times\AA\to[0,1]\}$

        \item (Reward Perturbation) 
        Suppose $\tilde{\RR} = \{ \tilde{r} :  \exists h: \SS\to \R, s.t., |r(s,a) + \E_{s'|s,a}[h(s)] - h(s) - \tilde{r}(s,a)| \leq \epsilon', \forall s\in\SS, a\in\AA\}$.  If $d^{\pi^*} \ll \mu$, then $\mu$ is $\frac{1-\gamma}{2 \epsilon'}$-robust
        \begin{align*}
         J(\pi^*) - J(\pi) 
         &= J(\pi^*) - \tilde{J}(\pi^*) + \tilde{J}(\pi^*) - \tilde{J}(\pi^\dagger) + \tilde{J}(\pi^\dagger) + \tilde{J}(\pi) - \tilde{J}(\pi) -  J(\pi) \\
         &\leq \frac{2 \epsilon'}{1-\gamma} + \delta
    \end{align*} 

        \item \todo{} (Forward Invariant States)
    \end{itemize}
\end{remark}


\todo{Need to talk about how the definition below relates to pessimism}
\begin{definition}[Admissible Offline RL Algorithm]
    For $\tilde{r}\in\tilde{\RR}$, consider an MDP $\tilde{\MM}=(\SS,\AA,\tilde{r},P,\gamma)$. %and a state-action distribution $\mu\in\Delta(\SS\times\AA)$. 
    For $R\geq 0$, we say an offline RL algorithm  $Algo$  is \emph{$R$-admissible} with respect to $\tilde{\RR}$, if for any $\tilde{r} \in\tilde{\RR}$, given an offline dataset of $\tilde{\MM}$ sampled on $\mu$,
    %$\tilde{\DD} \coloneqq \{ (s,a,r^\star,s') | (s,a) \sim \mu, r^\star = r^\star(s,a), s' \sim P(\cdot |s,a) \} $    
     $Algo$  learns a policy $\hat{\pi}$ satisfying the following with high probability:  for any policy $\pi\in\Pi$,
    \begin{align*}
        \max_{\bar{r} \in \RR_\mu^R(\tilde{r})} V_{\bar{r}}^\pi(d_0) - V_{\bar{r}}^{\hat{\pi}}(d_0) \leq \EE(\pi, \mu)
    \end{align*}
    where $\EE(\pi, \mu)$ is a regret upper bound such that $\EE(\pi, \mu) = o(1)$ if $d^\pi \ll \mu$ and 
    \begin{align}
        \RR_\mu^R(\tilde{r}) \coloneqq \left\{ \bar{r}: \bar{r}(s,a) = \tilde{r}(s,a), \forall (s,a) \in \supp{\mu} \textrm{ and }
        \bar{r}(s,a) \in  \left[-R, 1 \right], \forall (s,a) \in\SS\times\AA
        \right\}.
    \end{align}
    
\end{definition}

\chingan{Give examples: Show if we crank up the degree of pessimism, the algorithm would be admissible. }


% \begin{assumption} \label{as:data assumption}
%     The data generation distribution $\mu$ is $\frac{1}{\epsilon}$-robust with respect to $\tilde{\RR}$. In addition, for any $\tilde{r} \in \tilde{\RR}$, the constrained MDP $\CC_\mu(\tilde{r}) \coloneqq   \CC(\SS,\AA, \tilde{r},c_\mu,P,\gamma)$ in \cref{def:distribution robustness} has a sensitivity function $\sensitivity{\delta}{\CC_\mu(\tilde{r})} \leq R \delta$ for some $R<\infty$.
% \end{assumption}

% \begin{theorem}
%     Under \cref{as:data assumption}, consider an offline RL algorithm $Algo$ that is $(R+1)$-admissible with respect to $\tilde{\RR}$. 
%     Then for \emph{any} $\tilde{r}\in\tilde{\RR}$, with high probability, the policy $\hat{\pi}$ learned by $Algo$ from the dataset $\tilde{\DD} \coloneqq \{ (s,a,\tilde{r},s') | (s,a) \sim \mu, \tilde{r} = \tilde{r}(s,a), s' \sim P(\cdot |s,a) \} $ satisfies
%     \begin{align*}
%         J(\pi^*) - J(\hat\pi) \leq \epsilon + o(1)
%     \end{align*}
% \end{theorem}


\begin{assumption} \label{as:data assumption}
\mbox{}
\begin{enumerate}
        \item The data generation distribution $\mu$ is $\frac{1}{\epsilon}$-robust with respect to $\tilde{\RR}$.
        \item For any $\tilde{r} \in \tilde{\RR}$, the constrained MDP $\CC_\mu(\tilde{r}) \coloneqq   \CC(\SS,\AA, \tilde{r},c_\mu,P,\gamma)$ in \cref{def:distribution robustness} has a sensitivity function $\sensitivity{\delta}{\CC_\mu(\tilde{r})} \leq  K$ for some $K<\infty$ and $\lim_{\delta\to0^+} \kappa(\delta) = 0$.        
    \end{enumerate}     
\end{assumption}

The assumption on the convergence of $\kappa(\delta)$ to zero is to rule out some unrealistic edge cases of combination $\tilde{\RR}$ and $P$.


\begin{theorem}\label{th:performance guarantee}
    Under \cref{as:data assumption}, consider an offline RL algorithm $Algo$ that is $\frac{K}{\delta}$-admissible with respect to $\tilde{\RR}$. 
    Then for \emph{any} $\tilde{r}\in\tilde{\RR}$, with high probability, the policy $\hat{\pi}$ learned by $Algo$ from the dataset $\tilde{\DD} \coloneqq \{ (s,a,\tilde{r},s') | (s,a) \sim \mu, \tilde{r} = \tilde{r}(s,a), s' \sim P(\cdot |s,a) \} $ has performance guarantee
    \begin{align*}
        J(\pi^*) - J(\hat\pi) &\leq  \epsilon + O(\iota) %\\
        %V_{c_\mu}^{\hat\pi}(d_0) & \leq \iota
    \end{align*}
    and safety guarantee
    \begin{align*}
         (1-\gamma) \sum_{t=0}^\infty \gamma^t \mathrm{Prob}\left( \exists \tau\in[0,t] s_\tau \notin \supp{\mu}  | \hat{\pi}  \right)  \leq \iota
    \end{align*}
    where $\iota \coloneqq \delta + \sensitivity{\delta}{\CC_\mu(\tilde{r})} + o(1)$ and $o(1)$ denotes a term that vanishes as the dataset size becomes infinite.
\end{theorem}

% \begin{proof}
% We derive a lower bound of $ V_{c_\mu}^{\hat\pi}(d_0)$:
% \begin{align*}
%      V_{c_\mu}^{\hat\pi}(d_0) 
%      &= \sum_{t=0}^\infty  \gamma^t \E_{d_t^{\hat{\pi}}}[\one[ \mu(s,a)= 0]]\\
%      &\geq \sum_{t=0}^H \gamma^t \E_{d_t^{\hat{\pi}}}[\one[ \mu(s,a)= 0]]\\
%      &\geq \sum_{t=0}^H \E_{d_t^{\hat{\pi}}}[\one[ \mu(s,a)= 0]] - \sum_{t=0}^H (1-\gamma^t)   \\
%      &\geq \sum_{t=0}^H \E_{d_t^{\hat{\pi}}}[\one[ \mu(s,a)= 0]] - H + \frac{1-\gamma^H }{1-\gamma}  \\
%      &= \sum_{t=0}^H \E_{d_t^{\hat{\pi}}}[\one[ \mu(s,a)= 0]] + \frac{-\gamma^H }{1-\gamma}  
% \end{align*}

%     %(1+x)^n \leq \frac{1}{1-nx}
%     \begin{align*}
%         \gamma^H = (1-1+\gamma)^{\frac{1}{1-\gamma}} \leq \frac{1}{1+\frac{1}{1-\gamma}(1-\gamma)} \leq \frac{1}{2}
%     \end{align*}

%     \begin{align*}
%         \gamma^H = (1-1+\gamma)^{H} \leq \frac{1}{1+ H(1-\gamma)} 
%     \end{align*}

%     \begin{align*}
%         H  - \frac{1-\gamma^H }{1-\gamma} 
%         \leq H  - \frac{1- \frac{1}{1+ H(1-\gamma)}  }{1-\gamma} 
%         \leq H  - \frac{1}{1-\gamma}  + \frac{1}{(1+ H(1-\gamma))(1-\gamma)}
%     \end{align*}
% \end{proof}


\chingan{From here, show a corollary that offline RL is doubly robust and safe.}
\begin{proof}[Proof of \cref{th:performance guarantee}]
Below we prove by first showing $\hat{\pi} \in  \Pi_\omega(\CC_\mu(\tilde{r}))$ with $\omega = \delta + \sensitivity{\delta}{\CC_\mu(\tilde{r})} $ and then deriving the final performance guarantee using the robustness assumption.
%
To this end, we introduce some extra notations.  Given $\CC_\mu(\tilde{r})$, we define a perturbed constrained MDP problem: 
%\begin{align*}
 $   \max_\pi  V_{\tilde{r}}^\pi (d_0), \textrm{s.t.} V_{c_\mu}^\pi(d_0) \leq \delta$
%\end{align*}$
and its Lagrangian $ \LL_\delta(\pi, \lambda) \coloneqq V_{\tilde{r}}^\pi(d_0) - \lambda ( V_{c_\mu}^\pi(d_0) - \delta)$, where $\lambda\geq0$ denotes the Lagrange multiplier. Let $\pi_\delta^\dagger$ and $\lambda_\delta^\dagger$ denote the optimal policy and Lagrange multiplier of this perturbed constrained MDP, and recall the optimal policy to the unperturbed constrained MDP $\CC_\mu(\tilde{r})$ is denoted as $\pi^\dagger$. 
%
Finally we define a shorthand $r^\dagger (s,a) \coloneqq \tilde{r}(s,a) - (\lambda_\delta^\dagger+1) c_\mu(s,a)$. 


% To show $\hat{\pi} \in  \Pi_\delta(\CC_\mu(\tilde{r}))$, 
Now we bound the regret and the constraint violation of $\hat{\pi}$ in the constrained MDP $\CC_\mu(\tilde{r})$. The following holds for any $\delta\geq 0$. For the regret, we can derive 
\begin{align*}
    V_{\tilde{r}}^{\pi^\dagger}(d_0) - V_{\tilde{r}}^{\hat\pi}(d_0) 
    % & =   V_{\tilde{r}}^{\pi^\dagger}(d_0) - \lambda^\dagger  V_{c_\mu}^{\pi^\dagger}(d_0)  - V_{\tilde{r}}^{\hat\pi}(d_0) \\
    &= V_{\tilde{r}}^{\pi^\dagger}(d_0) - (\lambda_\delta^\dagger+1)  V_{c_\mu}^{\pi^\dagger}(d_0)  - V_{\tilde{r}}^{\hat\pi}(d_0) \\
    &\leq  V_{\tilde{r}}^{\pi^\dagger}(d_0) - (\lambda_\delta^\dagger+1)  V_{c_\mu}^{\pi^\dagger}(d_0) - V_{\tilde{r}}^{\hat\pi}(d_0) + (\lambda_\delta^\dagger+1) V_{c_\mu}^{\hat{\pi}}(d_0)\\
    &=  V_{r^\dagger}^{\pi^\dagger}(d_0) - V_{r^\dagger}^{\hat\pi}(d_0) 
\end{align*}
 On the other hand, for the constraint violation, we can derive
\begin{align*}
    V_{c_\mu}^{\hat\pi}(d_0) &= (V_{c_\mu}^{\hat\pi}(d_0) - \delta) + \delta\\
    &= (\lambda_\delta^\dagger + 1) (V_{c_\mu}^{\hat\pi}(d_0) -\delta) - \lambda_\delta^\dagger (V_{c_\mu}^{\hat\pi}(d_0) - \delta) + \delta\\
    &= - V_{\tilde{r}}^{\hat\pi}(d_0) + (\lambda_\delta^\dagger + 1) (V_{c_\mu}^{\hat\pi}(d_0)-\delta) + V_{\tilde{r}}^{\hat\pi}(d_0) - \lambda_\delta^\dagger (V_{c_\mu}^{\hat\pi}(d_0) - \delta) + \delta\\
    &= \LL_\delta (\hat\pi, \lambda_\delta^\dagger) - \LL_\delta(\hat\pi, \lambda_\delta^\dagger+1) + \delta\\
    % &\leq \LL_\delta(\pi_\delta^\dagger, \lambda_\delta^\dagger ) - \LL_\delta(\hat\pi, \lambda_\delta^\dagger+1) + \delta\\
    &\leq \LL_\delta(\pi_\delta^\dagger, \lambda_\delta^\dagger+1) - \LL_\delta(\hat\pi, \lambda_\delta^\dagger+1) + \delta\\
    &= V_{r^\dagger}^{\pi_\delta^\dagger}(d_0) - V_{r^\dagger}^{\hat\pi}(d_0) + \delta\\
    &\leq  V_{r^\dagger}^{\pi^\dagger}(d_0) - V_{r^\dagger}^{\hat\pi}(d_0) + \delta + \sensitivity{\delta}{\CC_\mu(\tilde{r})}  
\end{align*}
where the first inequality is due to that $(\pi_\delta^\dagger, \lambda_\delta^\dagger)$ is a saddle point to $\LL_\delta$, and the second inequality follows from
\begin{align*}
    V_{r^\dagger}^{\pi_\delta^\dagger}(d_0) 
    &=  V_{\tilde{r}}^{\pi_\delta^\dagger}(d_0) - (\lambda_\delta^\dagger +1)(V_{c_\mu}^{\pi_\delta^\dagger}(d_0) - \delta) \\
    &\leq V_{\tilde{r}}^{\pi_\delta^\dagger}(d_0) - (\lambda_\delta^\dagger +1)(V_{c_\mu}^{\pi^\dagger}(d_0) - \delta) \\
    &= V_{\tilde{r}}^{\pi^\dagger}(d_0) - (\lambda_\delta^\dagger +1)(V_{c_\mu}^{\pi^\dagger}(d_0) - \delta) 
    + \sensitivity{\delta}{\CC_\mu(\tilde{r})} 
\end{align*}




Next we bound on $V_{r^\dagger}^{\pi^\dagger}(d_0) - V_{r^\dagger}^{\hat\pi}(d_0)$.  
By \cref{lm:bound on dual variable} and \cref{as:data assumption}, we know $\lambda_\delta^\dagger \leq \frac{K}{\delta}$, so $r^\dagger(s,a) \in [-\frac{K}{\delta} , 1] $. This and the definition of $c_\mu$ together imply that $r^\dagger \in \RR_\mu(\tilde{r},\frac{K}{\delta})$. 
Since the offline RL algorithm $Algo$ is $\frac{K}{\delta}$-admissible, we have $V_{r^\dagger}^{\pi^\dagger}(d_0) - V_{r^\dagger}^{\hat\pi}(d_0) \leq \EE(\pi^\dagger, \mu)$. Finally, we use the fact that $\pi^\dagger$ by definition satisfies
 $d^{\pi^\dagger} \ll \mu$, so $\EE(\pi^\dagger,\mu)=o(1)$.
%
Thus, we have proved
\begin{align*}
    V_{\tilde{r}}^{\pi^\dagger}(d_0) - V_{\tilde{r}}^{\hat\pi}(d_0) &\leq o(1) \\
    V_{c_\mu}^{\hat\pi}(d_0)  &\leq  o(1) +  \delta + \sensitivity{\delta}{\CC_\mu(\tilde{r})}  
\end{align*}
That is, $\hat{\pi} \in  \Pi_\omega(\CC_\mu(\tilde{r}))$ with $\omega = \delta + \sensitivity{\delta}{\CC_\mu(\tilde{r})} $.

Finally, by $\frac{1}{\epsilon}$-robustness assumption on $\mu$, we have the performance bound.

To bound of out of support probability, we can write 
\begin{align*}
 V_{c_\mu}^{\hat\pi}(d_0) 
 &= \sum_{t=0}^\infty  \gamma^t  \E_{d_t^{\hat{\pi}}}[\one[ \mu(s,a)= 0]]\\
 &= (1-\gamma) \sum_{t=0}^\infty \gamma^t \left( \sum_{\tau=0}^t \E_{d_\tau^{\hat{\pi}}}[\one[ \mu(s,a)= 0]] \right) \\
 &\geq (1-\gamma) \sum_{t=0}^\infty \gamma^t \mathrm{Prob}\left( \exists \tau\in[0,t] s_\tau \notin \supp{\mu}  | \hat{\pi}  \right) 
 \end{align*}
 where second equality follows \citep{wagener2021safe}[Lemma 2].
\end{proof}


==> new_table.tex <==
\begin{table}[t]
\caption{ATAC table}
\label{tab:results}
\begin{center}
\begin{scriptsize}
\hspace*{-1.7in}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
\hline
Dataset & \multicolumn{4}{c}{ATAC with Different Reward Type} & \multicolumn{6}{c}{Baselines on Original Reward}\\
Dataset & Original reward & Constant 0 reward & Random reward 0 & Reward neg & Behavior & BC & CQL & TD3$+$BC & IQL & DT \\ 
\end{tabular}
\end{scriptsize}
\end{center}
\end{table}

\begin{table}[t]
\caption{CQL table}
\label{tab:results}
\begin{center}
\begin{scriptsize}
\hspace*{-1.7in}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
\hline
Dataset & \multicolumn{4}{c}{ATAC with Different Reward Type} & \multicolumn{6}{c}{Baselines on Original Reward}\\
Dataset & Original reward & Constant 0 reward & Random reward 0 & Reward neg & Behavior & BC & CQL & TD3$+$BC & IQL & DT \\ 
\end{tabular}
\end{scriptsize}
\end{center}
\end{table}

\begin{table}[t]
\caption{DT Table}
\label{tab:results}
\begin{center}
\begin{scriptsize}
\hspace*{-1.7in}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
\hline
Dataset & \multicolumn{4}{c}{ATAC with Different Reward Type} & \multicolumn{6}{c}{Baselines on Original Reward}\\
Dataset & Original reward & Constant 0 reward & Random reward 0 & Reward neg & Behavior & BC & CQL & TD3$+$BC & IQL & DT \\ 
\end{tabular}
\end{scriptsize}
\end{center}
\end{table}

\begin{table}[t]
\caption{IQL Table}
\label{tab:results}
\begin{center}
\begin{scriptsize}
\hspace*{-1.7in}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
\hline
Dataset & \multicolumn{4}{c}{ATAC with Different Reward Type} & \multicolumn{6}{c}{Baselines on Original Reward}\\
Dataset & Original reward & Constant 0 reward & Random reward 0 & Reward neg & Behavior & BC & CQL & TD3$+$BC & IQL & DT \\ 
\end{tabular}
\end{scriptsize}
\end{center}
\end{table}

\subsection{Experimental Setup}

We select hyperparameter for each reward type. For every environment and reward type, we try a small set of the most relevant hyperparameters and we run each combination with 2 evaluation seeds. We use the other hyperparameter choice suggested in the literature for D4RL with the original reward. We find the best hyperparameter using this evaluation and then run 5-10 seeds to compute confidence intervals.

We have $N=12$ environments and $K=4$ reward types. Let $L$ be the number of hyperparameter we try. Then total number of experiments are $NKL2 + NK5 = NK(2L + 5)$. We get $12 * 4 * (2 * 4 + 5) = 624$ jobs.

\begin{enumerate}
    \item CQL: Min CQL Weight $\{1, 2, 5, 8, 10\}$. Total number of experiments: $N\times K \times 5 \times 2$ ($600$ experiments) + $N \times K \times 5$ ($300$ experiments) = $900$ experiments
    \item ATAC: $\beta \in \{0.1, 1, 10, 100\}$: $N\times K \times 4 \times 2$ ($480$ experiments) and $N \times K \times 5$ ($300$ experiments) = $780$ experiments
    \item IQL: $\beta \in \{0.3, 3\}$ and $\tau \in \{0.7, 0.9\}$: $N\times K \times 4 \times 2$ ($480$ experiments) and $N \times K \times 5$ ($300$ experiments) = $780$ experiments
    \item DT: Learning rate and batch size. Unclear if we are doing any search. Evaluation is $N\times K \times 5$ = $300$ experiments.
\end{enumerate}



==> table.tex <==
\begin{table}[t]
\caption{TODO}
\label{tab:results}
\begin{center}
\begin{scriptsize}
\hspace*{-1.7in}
\begin{tabular}{c|c|c|c|c|c||c|c|c|c|c|c|c}
\hline
Dataset & reward rand & reward 1 & reward 0 & reward -1 & reward neg & Behavior & BC & ATAC & CQL & TD3$+$BC & IQL & DT \\ 
\hline
hopper-rand & \textbf{31.5} & \textbf{31.7} & \textbf{32.0} & \textbf{31.6} & \textbf{31.6} & 1.2 & 9.8 & 17.5 & 10.8 & 11.0 & - & - \\ 
\hline
hopper-med & \textbf{94.0} & \textbf{94.5} & \textbf{94.7} & \textbf{96.9} & \textbf{92.4} & 44.2 & 29.0 & 85.6 & 86.6 & \textbf{99.5} & 66.3 & 67.6 \\ 
\hline
hopper-med-replay & 65.0 & 82.5 & 68.5 & 84.5 & 33.5 & 14.9 & 11.8 & \textbf{102.5} & 48.6 & 31.4 & \textbf{94.7} & 82.7 \\ 
\hline
hopper-med-exp & 63.9 & 92.4 & \textbf{110.1} & \textbf{104.7} & 91.0 & 64.7 & \textbf{111.9} & \textbf{111.9} & \textbf{111.0} & \textbf{112.2} & 91.5 & 107.6 \\ 
\hline
hopper-exp & \textbf{111.2} & \textbf{111.1} & \textbf{111.2} & \textbf{110.8} & \textbf{111.1} & \textbf{108.5} & - & - & - & - & - & - \\ 
\hline
walker2d-rand & \textbf{6.4} & 5.5 & 6.0 & \textbf{6.8} & \textbf{6.6} & 0.0 & 1.6 & \textbf{6.8} & \textbf{7.0} & 1.4 & - & - \\ 
\hline
walker2d-med & 78.9 & 76.7 & 76.6 & 77.4 & 72.6 & 62.0 & 6.6 & \textbf{89.6} & 74.5 & 79.7 & 78.3 & 74.0 \\ 
\hline
walker2d-med-replay & 70.8 & 70.1 & 58.4 & 71.7 & 54.8 & 14.8 & 11.3 & \textbf{92.5} & 32.6 & 25.2 & 73.9 & 66.6 \\ 
\hline
walker2d-med-exp & \textbf{109.5} & 93.5 & 85.7 & 95.1 & 73.0 & 82.6 & 6.4 & \textbf{114.2} & 98.7 & 101.1 & \textbf{109.6} & 108.1 \\ 
\hline
walker2d-exp & \textbf{108.1} & \textbf{108.0} & \textbf{108.2} & \textbf{108.4} & \textbf{107.7} & \textbf{107.1} & - & - & - & - & - & - \\ 
\hline
halfcheetah-rand & 2.3 & 2.3 & 2.2 & 2.3 & 2.2 & -0.1 & 2.1 & 3.9 & \textbf{35.4} & 10.2 & - & - \\ 
\hline
halfcheetah-med & 42.7 & 42.9 & 42.7 & 42.9 & 40.1 & 40.6 & 36.1 & \textbf{53.3} & 44.4 & 42.8 & 47.4 & 42.6 \\ 
\hline
halfcheetah-med-replay & 37.3 & 39.6 & 36.6 & 37.8 & 40.1 & 27.1 & 38.4 & \textbf{48.0} & \textbf{46.2} & \textbf{43.3} & \textbf{44.2} & 36.6 \\ 
\hline
halfcheetah-med-exp & 56.5 & 48.8 & 47.6 & 56.9 & 40.4 & 64.3 & 35.8 & \textbf{94.8} & 62.4 & \textbf{97.9} & 86.7 & 86.8 \\ 
\hline
halfcheetah-exp & \textbf{91.8} & \textbf{93.2} & \textbf{92.9} & \textbf{93.9} & \textbf{93.0} & \textbf{88.1} & - & - & - & - & - & - \\ 
\hline
\end{tabular}
\hspace*{-1.7in}
\end{scriptsize}
\end{center}
\end{table}

\begin{table}[t]
\caption{Total number of trajectories, number of full trajectories, and average trajectory length in each D4RL dataset.}
\label{tab:num_trajs}
\begin{center}
\begin{tabular}{c|c|c|c}
\hline
Dataset & Total Trajs & Full Trajs & Avg Traj Len\\
\hline
hopper-random-v2 & 45240 & 1 & 22.10\\
\hline
hopper-medium-v2 & 2187 & 2 & 457.25\\
\hline
hopper-medium-replay-v2 & 2041 & 402 & 196.96\\
\hline
hopper-medium-expert-v2 & 3214 & 940 & 622.25\\
\hline
walker2d-random-v2 & 48908 & 1 & 20.45\\
\hline
walker2d-medium-v2 & 1191 & 678 & 839.63\\
\hline
walker2d-medium-replay-v2 & 1093 & 302 & 276.30\\
\hline
walker2d-medium-expert-v2 & 2191 & 1677 & 912.82\\
\hline
halfcheetah-random-v2 & 1000 & 1000 & 1000.00\\
\hline
halfcheetah-medium-v2 & 1000 & 1000 & 1000.00\\
\hline
halfcheetah-medium-replay-v2 & 202 & 202 & 1000.00\\
\hline
halfcheetah-medium-expert-v2 & 2000 & 2000 & 1000.00\\
\hline
ant-random-v2 & 5822 & 573 & 171.76\\
\hline
ant-medium-v2 & 1203 & 825 & 831.26\\
\hline
ant-medium-replay-v2 & 485 & 302 & 622.68\\
\hline
ant-medium-expert-v2 & 2237 & 1788 & 894.03\\
\end{tabular}
\end{center}
\end{table}
